TrAME: Trajectory-Anchored Multi-View Editing for Text-Guided 3D Gaussian Splatting Manipulation

Despite significant strides in the field of 3D scene editing, current methods encounter substantial challenge, particularly in preserving 3D consistency in multi-view editing process. To tackle this challenge, we propose a progressive 3D editing strategy that ensures multi-view consistency via a Trajectory-Anchored Scheme (TAS) with a dual-branch editing mechanism. Specifically, TAS facilitates a tightly coupled iterative process between 2D view editing and 3D updating, preventing error accumulation yielded from text-to-image process. Additionally, we explore the relationship between optimization-based methods and reconstruction-based methods, offering a unified perspective for selecting superior design choice, supporting the rationale behind the designed TAS. We further present a tuning-free View-Consistent Attention Control (VCAC) module that leverages cross-view semantic and geometric reference from the source branch to yield aligned views from the target branch during the editing of 2D views. To validate the effectiveness of our method, we analyze 2D examples to demonstrate the improved consistency with the VCAC module. Further extensive quantitative and qualitative results in text-guided 3D scene editing indicate that our method achieves superior editing quality compared to state-of-the-art methods. We will make the complete codebase publicly available following the conclusion of the review process.

==> bios.tex <==
\begin{IEEEbiography}
[{\includegraphics[width=0.8in,height=1in,clip,keepaspectratio]{bios/chaofanluo.jpeg}}]{Chaofan Luo} received his B.E. degrees from Tianjin University in Tianjin, China. His research interests lies in 3D graphics, generative models, and machine learning. Currently, he is a graduate student in School of Information Science and Technology, University of Science and Technology of China, Anhui, China.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=0.8in,height=1in,clip,keepaspectratio]{bios/DonglinDi.png}}]{Donglin Di} received his B.E. and M.S. degrees from the Harbin Institute of Technology in Harbin, China. His research interests encompass computer vision, generative models, and machine learning. Currently, he is a senior algorithm engineer and the leader of the Digital Avatar Department at Space AI in Li Auto, based in Beijing, China.
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=0.8in,height=1in,clip,keepaspectratio]{bios/xunyang.jpeg}}]{Xun Yang} received the Ph.D. degree in signal and information processing from Hefei University of Technology, Hefei, China, in 2017.
He is currently a Professor with the Department of Electronic Engineering and Information Science, University of Science and Technology of China (USTC), Hefei, China. From 2015 to 2017, he visited the University of Technology Sydney (UTS), Sydney, Australia, as a Joint Ph.D. Student. His current research interests include information retrieval, cross-media analysis and reasoning, and computer vision.
Dr. Yang served as the Area Chair for the ACM Multimedia 2022. He also serves as an Associate Editor for the journal of IEEE Transactions on Big Data.
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=0.8in,height=1in,clip,keepaspectratio]{bios/YongjiaMa.png}}]{Yongjia Ma} received his B.E. degree from Central South University in Changsha, China, and his M.S. degree from Xi'an Jiaotong University in Xi'an, China. His research interests include neural rendering, generative models, and machine learning. Currently, he is an algorithm engineer in the Digital Avatar Department at Space AI in Li Auto, based in Beijing, China.
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=0.8in,height=1in,clip,keepaspectratio]{bios/ZhouXue.jpeg}}]{Zhou Xue} received the B.E. degree in information engineering from Beijing University of Posts and Telecommunications, the M.S. degree in automation from Tsinghua University and the Ph.D degree in computer and communication sciences from the Swiss Federal Institute of Technology Lausanne (EPFL). He is currently a system architect/researcher with Kunlun Digital Technology Corporation of China National Petroleum Corporation. His research interests include 3D vision, generative models and AR/VR.
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=0.8in,height=1in,clip,keepaspectratio]{bios/WeiChen.jpeg}}]{Wei Chen} received the Ph.D. degree in signal and information processing from the Beijing University of Posts and Telecommunications, Beijing, China, in 2011. Since 2021, He has been the Chief Scientist with Smart cockpit department of Li Auto, which is a leader in China’s new energy vehicle market. His research interests include multi-modal large language model, speech recognition and synthesis, computer vision.
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=0.8in,height=1in,clip,keepaspectratio]{bios/XiaofeiGou.jpeg}}]{Xiaofei Gou} is the head of Li Auto's smart space, focusing on the research and development of space interaction in smart cockpit, including hardware, operating system and AI.
\end{IEEEbiography}


\begin{IEEEbiography}
[{\includegraphics[width=0.8in,height=1in,clip,keepaspectratio]{bios/yebinliu.jpeg}}]{Yebin Liu} (Member, IEEE) received the BE degree from the Beijing University of Posts and Telecommunications, China, in 2002, and the PhD degree from the Automation Department, Tsinghua University, Beijing, China, in 2009. He is currently a professor with Tsinghua University. His research areas include computer vision, computer graphics and computational photography.
\end{IEEEbiography}

